A Generative Modeling Approach to Limited Channel ECG Classification

Processing temporal sequences is central to a variety of applications in health care, and in particular multi-channel Electrocardiogram (ECG) is a highly prevalent diagnostic modality that relies on robust sequence modeling. While Recurrent Neural Networks (RNNs) have led to significant advances in automated diagnosis with time-series data, they perform poorly when models are trained using a limited set of channels. A crucial limitation of existing solutions is that they rely solely on discriminative models, which tend to generalize poorly in such scenarios. In order to combat this limitation, we develop a generative modeling approach to limited channel ECG classification. This approach first uses a Seq2Seq model to implicitly generate the missing channel information, and then uses the latent representation to perform the actual supervisory task. This decoupling enables the use of unsupervised data and also provides highly robust metric spaces for subsequent discriminative learning. Our experiments with the Physionet dataset clearly evidence the effectiveness of our approach over standard RNNs in disease prediction.

==> related.tex <==
\begin{itemize}
	\item RNNs in medical data analysis
	\item State-of-the-art papers in this space
	\item Existing approaches for limited-channel data
	\item To the best of our knowledge, this is the first approach to employ a generative modeling approach to limited channel analysis
\end{itemize}
%The core idea of our setup is
%to extract a diverse set of features from the sequence of
%heartbeats in an ECG record to be used as input features
%to an ensemble of RNNs. We blend the individual models’
%predictions into a per-class classification score using a
%multilayer perceptron (MLP) with a softmax output layer. 
%As part of preprocessing they do segmentation to reduce timesteps from 9000 to 33, where qrs (pan-tomkins) is detected. Each sample is now a 0.66s window around R-peak. After segmentation, they extract features such as: RR, relative wavelet energy (rwe), total wavelet energy (twe), R, Q amplitude, qrs duration, and wavelet entropy. They further train stacked auto-enco on heartbeats and another on their wavelet coeffs, to get 2 embedded representations and add them to the computed features. [Beat by Beat:
%Classifying Cardiac Arrhythmias with Recurrent Neural Networks] - main thing = using soft attention in RNN for interpretability, and custom feature extraction from ecg literature, fewer hyperparams. F1-score 0.79 on CinC challenge, and class-wise 0.90, 0.79 and 0.68 for normal rhythms, AF and other arrhythmias.
%
%Recently, Rajpurkar et al. proposed
%a 34-layer convolutional neural network (CNN) to
%reach cardiologist-level performance in classifying a large
%set of arrhythmias from mobile cardiac event recorder data. They used FCN, data from mobile single channel alive cor. [Rajpurkar, cardiologist level]
%
%[beat by beat] claims to be state-of-the-art than [rajpurkar] by having fewer training params.



